Eigenperiods and the moduli of points in the line

We study the period map of configurations of n points on the projective line constructed via a cyclic cover branching along these points. By considering the decomposition of its Hodge structure into eigenspaces, we establish the codimension of the locus where the eigenperiod map is still pure. Furthermore, we show that the period map extends to the divisors of a specific moduli space of weighted stable rational curves, and that this extension satisfies a local Torelli map along its fibers.

==> 1-Intro-Old01.tex <==
\section{Introduction}
Understanding the connection between geometric and Hodge-theoretic compactifications of moduli spaces of varieties is a central quest within algebraic geometry. In particular, attention is given to the role of these compactifications in expanding a given period map and to Torelli-type results for singular varieties. 
A classical example of such results is due to 
Deligne and Mostow \cite{DM86}. They showed that certain geometric compactifications of the moduli space for up to 12 partially labeled points in $\mathbb{P}^1$, constructed via Geometric Invariant Theory, are isomorphic to a Hodge-theoretic compactification of the image of their period domain - the Baily-Borel compactification. This result has been further extended to isomorphisms among other geometric and Hodge-theoretic  compactifications of such moduli spaces of points \cite{gallardo2021geometric}.

Yet, it remains unknown whether the Deligne-Mostow results can be partially generalized to an arbitrary number of points. To understand the difficulties, let us recall the construction of the period map for $n$ points in $\mathbb{P}^1$. It begins with a cyclic cover $C$ of degree $d$ branching along these points. The Galois group of this finite cover  lifts to both the cohomology of and the Hodge structure on $C$. Thus, the action of the Galois group induces an eigenspace decomposition on $H^1(C)$ indexed by an integer $k$.  One can restrict the Hodge structure of $C$ to the $k$-th eigenspace to construct a potential eigenperiod map characterized by the data $(d,k)$. Two important problems arise: for an arbitrary number of points the potential eigenperiod map is not dominant and the monodromy representation may not even be discrete. Nowadays, it is understood that many interesting period maps are dominant into their period domains.  McMullen described conditions on $(d,k)$ ensuring that the associated monodromy representation is discrete, see Theorem \ref{thm:Mcmullen} and Table \ref{tab:ancestorCases}. Therefore, it is possible to define a family of eigenperiods that contain and generalize the Deligne-Mostow cases, as seen in Proposition \ref{prop:EigenPeriodM0n}.

In our first result, we consider an extension of eigenperiod maps mentioned above. 
This is possible because there is a geometric smooth normal crossing compactification  of the moduli of $n$ labelled points on the line known as $\overline{M}_{0,n}$. In addition, there is a Hodge-theoretical compactification of the period domain known as Kato and Usui's compactification
\cite{KU08}, which aligns with the toroidal compactification introduced by \cite{AMRT10} in the classical case. For our period domains, the construction of Kato-Usui's space denoted  as 
$(\Gamma^{\mathrm{nm}}_{n,d,k}\backslash D_{n,d,k})_{\Sigma}$
depends on the selection of an admissible fan $\Sigma$, and it may require a finite cover extension induced by selecting a neat subgroup $\Gamma^{\mathrm{nm}}_{n,d,k} \subset \Gamma_{n,d,k}$. 
\footnote{We will change the following to proposition. We add text that explain the main result is the Prop 1.2 which will become a theorem. }

\begin{proposition}
\label{prop:extension}
Let $n \geq 5$ and $k/d$ be as specified in Table \ref{tab:ancestorCases}, and suppose that $ \gcd(d,n-1)=1$ holds. There exist an eigenperiod map coming from the family of cyclic cover of $\mathbb{P}^1$ branched over marked points, see Proposition \ref{prop:EigenPeriodM0n},      
\[
\Phi_{n,d,k}:M_{0,n} \to
\Gamma_{n,d,k}\backslash D_{n,d,k}
\]
such that 
\begin{itemize}
    \item[(i)]  There exists a maximal partial compactification $M_{0,n}^{\mathrm{pr}} \subset \overline{M}_{0,n}$ over which $\Phi_{n,d,k}$ extends, that is 
    \[
    \Phi_{n,d,k}:M_{0,n}^{\mathrm{pr}} \to
    \Gamma_{n,d,k}\backslash D_{n,d,k}.
    \]
    \item[(ii)]
    The space $M_{0,n}^{\mathrm{pr}}$ is characterized by the following property: For any $p\in \overline{M}_{0,n}$, $p\in M_{0,n}^{\mathrm{pr}}$ if and only if for any $1$-dimensional contractible neighboorhood $p\in U\subset \overline{M}_{0,n}$ with $U-\{p\}\subset M_{0,n}$, the variation of Hodge structure associated to $\Phi_{n,d,k}|_{U-\{p\}}$ has finite monodromy. 
    
\end{itemize}
\end{proposition}
We remark the necessity of the condition $\mathrm{gcd}(d, n-1)=1$: It secures the existence of a branched covering map $\mathcal{C}\rightarrow \mathbb{P}^1$ of generic degree $d$, and the ramification loci is the union of $n$ distinct points on $\mathbb{P}^1$, each of which has ramification degree $d-1$, see \cite[Sec. 3]{McM13}.

To determine the space $M_{0,n}^{\mathrm{pr}}$ based on the property (ii), there are two methods. One way is through the geometric perspective: In the spirit that $n$ points on $\mathbb{P}^1$ gives a cyclic $d$-cover branched over these points, $M_{0,n}^{\mathrm{pr}}$ is the sub-moduli space of $\overline{M}_{0,n}$ producing stable curves of compact type, i.e., whose dual graph is a tree. Another way is using the Hodge-theoretic method to describe the singularities of the curve which we will treat below. We say that $M_{0,n}^{\mathrm{pr}}$ is the pure locus because the limiting mixed Hodge structures (LMHS) obtained from the local period maps over $\Delta$ around $p \in M_{0,n}^{\mathrm{pr}}$ are pure as a direct consequence of finite local monodromy. We will give precise combinatorial conditions for a point $p\in \overline{M}_{0,n}$ to locate in the pure locus. Moreover, we calculate the codimension of the complement of the ``pure" loci as established in Proposition 
\ref{prop:extension} within a pertinent GIT compactification, see Table \ref{tab:ancestorCases}.
\newpage
\begin{theorem}\label{thm:codimensions}
Let $n, k$ and $d$ be as in Proposition \ref{prop:extension}, then $M^{pr}_{0,n}$ is explicitly given by 
\begin{align*}
M^{pr}_{0,n} = 
\overline{M}_{0,n}
\setminus
\bigcup_{ I \notin \mathcal{I}^{pr} } 
D_{I,I^c}
&& 
\mathcal{I}^{pr} = 
\{ I \; : \;
k\min\{ |I|, |I^c| \} \not\equiv 0 \text{mod}(d) 
\; \}.
\end{align*}
Moreover, 
let
$
\overline{M}^{\mathrm{\mathrm{\mathrm{GIT}}}}_{0, \mathbf{w}} $ be the GIT compactification relative to the weights
$ \mathbf{w} = (\frac{2}{n}, ..., \frac{2}{n})$
if $d|n$, and 
$
\mathbf{w} = 
(\frac{1}{n-1}+\epsilon, ..., \frac{1}{n-1}+\epsilon, 1-(n-1)\epsilon )
$
if  $d \nmid n$ and 
$\gcd(d,n-1)=1$. 
and the reduction morphism 
$
\pi: \overline{M}_{0,n} \longrightarrow \overline{M}^{\mathrm{\mathrm{\mathrm{GIT}}}}_{0, \mathbf{w}} 
$, then it holds that 
\begin{align*}
\cod\left( 
\overline{M}^{\mathrm{\mathrm{\mathrm{GIT}}}}_{0, \mathbf{w}} 
\setminus
\pi(M^{\mathrm{pr}}_{0,n})
\right) =:H(n,d,k).
\end{align*}
Where if $d|n$, then 
\begin{align*}
H(n,d,k) = \left\{ \begin{array}{rcl}
 \frac{d}{\mathrm{gcd}(k,d)}-1 & \mbox{\textrm{if}}
& \textrm{gcd}(k,d)>\frac{2d}{n} \\ n-3 & \mbox{\textrm{if}} & \textrm{gcd}(k,d)=\frac{2d}{n} \\ \infty & \mbox{\textrm{if}} & \textrm{gcd}(k,d)<\frac{2d}{n}
\\
\end{array}\right.    
\end{align*}
On the other hand, if $d\nmid n$ and $\gcd(d,n-1)=1$, then 
\begin{align*}
H(n,d,k) = \left\{ \begin{array}{rcl}
 \frac{d}{\mathrm{gcd}(k,d)}-1 & \mbox{\textrm{if}}
& \textrm{gcd}(k,d)>\frac{d}{n-2} \\ n-3 & \mbox{\textrm{if}} & \textrm{gcd}(k,d)=\frac{d}{n-2} \\ \infty & \mbox{\textrm{if}} & \textrm{gcd}(k,d)<\frac{d}{n-2}
\\
\end{array}\right.    
\end{align*}
Note that if the codimension is infinite, it implies that $\pi(M^{\mathrm{pr}}_{0,n})=\overline{M}^{\mathrm{\mathrm{\mathrm{GIT}}}}_{0, \mathbf{w}}$.
\end{theorem}
To prove Theorem \ref{thm:codimensions}, we analyze in Section ~\ref{sec:PureLocus} the eigenspectra of the degenerations parametrized by the partial compactification $M_{0,n}^{\mathrm{pr}}$. This perspective  extends Steenbrink's theory on the spectrum of hypersurface singularities, as seen in \cite{KL20}, \cite{castor2022remarks}. The proof is then completed by studying  the behavior of the LMHS arising from degenerations of eigenperiod maps, as detailed in Section
\ref{sec:ExtensionPureLocus}. 

To describe our following result, we recall that by Proposition \ref{prop:extension} and Kato-Usui theory \cite{KU08},  there exists a finite-index normal neat subgroup $\Gamma^{\mathrm{nm}}_{n,d,k}\leq \Gamma_{n,d,k}$, and a normalization of a finite cover $\overline{M}^{\mathrm{nm}}_{0,n} \to \overline{M}_{0,n}$ such that the lift of $\Phi_{n,d,k}$ admits a Kato-Usui-Toroidal type extension:
\begin{align*}
    \xymatrix{
    \Phi^{\mathrm{nm}}_{n,d,k}:   \overline{M}^{\mathrm{nm}}_{0,n}
    \ar@{.>}[r]& 
    \left( \Gamma^{\mathrm{nm}}_{n,d,k}\backslash D_{n,d,k} \right) 
    \bigsqcup_{N\in \Gamma^{\mathrm{nm}}_{n,d,k}\backslash \Sigma}(\Gamma_N\backslash B(N)).
    }
\end{align*}
in codimension one (here, $\Gamma_N$ denotes the stabilizer of $N$ in $\Gamma^{\mathrm{nm}}_{n,d,k}$.) Therefore, it is most interesting to understand the extended period map better.

For an even number $n$, there is a smooth geometric compactification, commonly known as Hassett's moduli spaces of weighted stable curves \cite{hassett2003moduli}, with a unique divisor $\mathcal{D}$ in  
$\overline{M}_{0,\mathbf{\frac{2}{n}} + \epsilon}/S_n$ that generically parametrizes a weighted stable curve described as follows: It is the union of two $\mathbb{P}^1$ components, each with $r$ distinct marked points glued at another nodal singularity. 
In an open locus $\mathcal{D}^{\circ} \subset \mathcal{D}$ on which the glueing point does not collide with any marked point on either components, we obtain a reduction map 
\begin{align*}
\mathcal{R}:& \mathcal{D}^{\circ} \longrightarrow \mathrm{Sym}^2(M_{0,r}/S_r)
\end{align*}
by disregarding the gluing points on each $\mathbb{P}^1$, see Equation \eqref{eq:R}.  By
the same argument as used for Proposition \ref{prop:extension}, we have a rational map 
$$
\xymatrix{
\overline{M}_{0,\mathbf{\frac{2}{n}} + \epsilon}^{nm}
\ar@{.>}[r]& 
(\Gamma^{\mathrm{nm}}_{n,d,k}\backslash D_{n,d,k})_{\Sigma}
}
$$
where $\overline{M}_{0,\mathbf{\frac{2}{n}} + \epsilon}^{nm}$ is a finite cover of $\overline{M}_{0,\mathbf{\frac{2}{n}} + \epsilon}/S_n$.  Our next result extends this rational map to the interior of the divisors $\mathcal{D}$, and shows that such an extension satisfies a local Torelli-type theorem. 
We denote the union of $M_{0,n}$ and all codimension one strata within $\overline{M}_{0,\mathbf{\frac{2}{n}} + \epsilon}$ 
as $\overline{M}^{\circ}_{0,\mathbf{\frac{2}{n}} + \epsilon} \subset \overline{M}_{0,\mathbf{\frac{2}{n}} + \epsilon}$. 
The selection of a neat subgroup $\Gamma^{\mathrm{nm}}_{n,d,k} \subset 
\Gamma_{n,d,k}$ induces a lift $\mathcal{D}^{\mathrm{nm},\circ}$ and $\mathcal{R}^{\mathrm{nm}}$ for both the divisor $\mathcal{D}^{\circ}$ and the map $\mathcal{R}$. 
In our case, $\Sigma$ is a polyhedral fan in $\mathrm{Lie}(U(r,s))$ with rays generated by the monodromy logarithm $N$ around each divisor $\mathcal{D}$. 
\begin{theorem}\label{thm:KU}
Let $(n,d,k)$ be as in Proposition \ref{prop:extension}(i) and with $n$ even. Then, there exists a finite-index normal neat subgroup $\Gamma^{\mathrm{nm}}_{n,d,k}\leq \Gamma_{n,d,k}$, and a normalization of a finite cover $\overline{M}^{\mathrm{nm},\circ}_{0,\mathbf{\frac{2}{n}} + \epsilon} \longrightarrow \overline{M}_{0,\mathbf{\frac{2}{n}} + \epsilon}^{\circ}/S_n$ such that:
\begin{enumerate}
    \item  The eigenperiod map
    $$
    \phi_{n,d,k} :M_{0,n}/S_n \longrightarrow 
    \Gamma_{n,d,k}\backslash D_{n,d,k}
    $$
    has a unique lift which admits a Kato-Usui type extension:
    \begin{align*}
    \xymatrix{
    \phi^{\circ}_{n,d,k}:   \overline{M}^{\mathrm{nm},\circ}_{0,\mathbf{\frac{2}{n}} + \epsilon}
    \ar[r]& 
    \left( \Gamma^{\mathrm{nm}}_{n,d,k}\backslash D_{n,d,k} \right) 
    \bigsqcup_{N\in \Gamma^{\mathrm{nm}}_{n,d,k}\backslash \Sigma}(\Gamma_N\backslash B(N)).
    }
    \end{align*}
where $\Gamma_N$ denotes the stabilizer of $N$ in $\Gamma^{\mathrm{nm}}_{n,d,k}$.
    \item For $k=1$, the restriction of $\phi^{\circ}_{n,d,k}$ to any fiber $\left( \mathcal{R}^{\mathrm{nm}} \right)^{-1}(x)$ is an immersion.
    i.e. the map is locally injective. 
\end{enumerate}
\end{theorem}
Our result includes all the Deligne-Mostow cases \cite{gallardo2021geometric} and some cases with $n>12$ that are not covered by Deligne-Mostow. The first statement is a consequence of the techniques employed in \cite[Sec. 3.3]{gallardo2021geometric}. The second part of the theorem follows from a study of the associated Abel-Jacobi map.


\subsection*{Acknowledgements}
We would like to thank Matt Kerr, Gregory Pearlstein, Nolan Schock and Yilong Zhang for insightful discussions and comments.  We are grateful for the working environments at the Department of Mathematics in Washington University in St. Louis, University of California, Riverside and  Duke University where this research was conducted.  
The second author is partially supported by the National Science Foundation under Grant No. DMS-2316749.
